A Fast Convergence Theory for Offline Decision Making

This paper proposes the first generic fast convergence result in general function approximation for offline decision making problems, which include offline reinforcement learning (RL) and off-policy evaluation (OPE) as special cases. To unify different settings, we introduce a framework called Decision Making with Offline Feedback (DMOF), which captures a wide range of offline decision making problems. Within this framework, we propose a simple yet powerful algorithm called Empirical Decision with Divergence (EDD), whose upper bound can be termed as a coefficient named Empirical Offline Estimation Coefficient (EOEC). We show that EOEC is instance-dependent and actually measures the correlation of the problem. When assuming partial coverage in the dataset, EOEC will reduce in a rate of $1/N$ where $N$ is the size of the dataset, endowing EDD with a fast convergence guarantee. Finally, we complement the above results with a lower bound in the DMOF framework, which further demonstrates the soundness of our theory.

==> lemmas/divergence_of_process.tex <==
\subsection{Divergence of Stochastic Processes}

\begin{align*}
    D_f(\mathbb{P}\Vert \mathbb{Q})\coloneqq \int_A f\Big(\frac{p(x)}{q(x)}\Big)q(x)d\nu(x)+f^\prime(\infty)\mathbb{P}(E\setminus A)
\end{align*}


==> lemmas/inverse_chain.tex <==
\begin{lemma}[Superadditivity for the Squared Hellinger Distance]
    \label{lemma:subadd-h}
    Let $\{(\Xcal_i, \Fcal_i)\}_{i\in[n]}$ be a sequence of measurable spaces, $\Xcal^{(i)}=\prod_{t=1}^i\Xcal_t$, and $\Fcal^{(i)}=\bigotimes_{t=1}^i\Fcal_i$.
    For each $i\in[n]$, let $\mathbb{P}^{(i)}(\cdot|\cdot)$ and $\mathbb{Q}^{(i)}(\cdot|\cdot)$ be probability kernels from $(\Xcal^{(i-1)}, \Fcal^{(i-1)})$ to $(\Xcal_i, \Fcal_i)$.
    Let $\mathbb{P}$ and $\mathbb{Q}$ be the laws of $\{X_i\}_{i\in[n]}$ under $X_i\sim\mathbb{P}^{(i)}(\cdot|\{X_t\}_{t\in[0, i-1]})$ and 
    $X_i\sim\mathbb{Q}^{(i)}(\cdot|\{X_t\}_{t\in[0, i-1]})$ respectively.
    Then it holds that
    \begin{align*}
        \HH(\mathbb{P}, \mathbb{Q})\le 10^2\log(n)\cdot\mathbb{E}_{\mathbb{P}}\Big[\sum_{i=1}^n \HH(\mathbb{P}(\cdot|\{X_t\}_{t\in[i-1]}), \mathbb{Q}(\cdot|\{X_t\}_{t\in[i-1]})\Big].
    \end{align*}
\end{lemma}




==> lemmas/r_simulation.tex <==
\subsection{Missing Proof of \Cref{theorem:refined-simulation}}
\label{subsection:r-sim}

\begin{theorem}[Refined Simulation Lemma]%
    \textcolor{red}{C. Mao-TODO: lack some constants}
    Given a sequential problem $(\Pcal, \Mcal, \Pi, \{\ell_h\}_{h\in[H]})$, for any $M, M^\prime\in\Mcal$ and $\pi\in\Pi$, we have that
    \begin{align*}
        &\quad\quad\Lcal(M, \pi)\\&\lesssim\Lcal(M^\prime, \pi)+\frac{1}{H}\sum_{h=0}^H\mathbb{E}_{\{X_{h^\prime}\}_{h^\prime\in[H]}\sim\Pcal(M, \pi)}\Big[\HH\Big(\Pcal_h(M, \pi|\{X_{h^\prime}\}_{h^\prime\in[h-1]}), \Pcal(M^\prime, \pi|\{X_{h^\prime}\}_{h^\prime\in[h-1]})\Big)\Big].
    \end{align*}
\end{theorem}

The process $\{X_h\}_{h\in[H]}$, probability measures $\Pcal(M, \pi)$ and $\Pcal(M^\prime, \pi)$ in \Cref{definition:s-p} satisfy the condition required in \Cref{lemma:subadd-h}, which means that 

\begin{align*}
    \HH(\Pcal(M, \pi), \Pcal(M^\prime, \pi))\le
    10^2\log(H)\cdot\mathbb{E}_{\{X_{h^\prime}\}_{h^\prime\in[H]}\sim\Pcal(M, \pi)}\Big[\sum_{i=1}^H \HH\big(\Pcal(M, \pi|\{X_t\}_{t\in[i-1]}), \Pcal(M^\prime, \pi|\{X_t\}_{t\in[i-1]})\big)\Big].
\end{align*}

By the change of measure property of the squared Hellinger distance, we have that 

\begin{align*}
    \Lcal(M, \pi)\le&3\Lcal(M^\prime, \pi)+4B\cdot\HH(\Pcal(M, \pi), \Pcal(M^\prime, \pi))\\\le&
    3\Lcal(M^\prime, \pi)+4B\cdot 10^2\log(H)\cdot\mathbb{E}_{\{X_{h^\prime}\}_{h^\prime\in[H]}\sim\Pcal(M, \pi)}\Big[\sum_{i=1}^H \HH\big(\Pcal(M, \pi|\{X_t\}_{t\in[i-1]}), \Pcal(M^\prime, \pi|\{X_t\}_{t\in[i-1]})\big)\Big]
\end{align*}

This completes the proof.

\textcolor{red}{C. Mao-TODO: Move this to ...}
Finally by the positiveness of the squared Hellinger distance and the definition of the coverage coefficient, we can conclude that 
\begin{align*}
    \Lcal(M, \pi)\le&3\Lcal(M^\prime, \pi)+4B\cdot\HH(\Pcal(M, \pi), \Pcal(M^\prime, \pi))\\\le&
    3\Lcal(M^\prime, \pi)+4BC\cdot 10^2\log(H)\cdot\mathbb{E}_{\{X_{h^\prime}\}_{h^\prime\in[H]}\sim\Pcal(M, \pi)}\Big[\sum_{i=1}^H \HH\big(\Pcal(M, \pi|\{X_t\}_{t\in[i-1]}), \Pcal(M^\prime, \pi|\{X_t\}_{t\in[i-1]})\big)\Big]
\end{align*}


==> lemmas/tightness.tex <==
\section{On The Tightness of The Bound}
\label{proof:tightness}

For a probability measure $\mathbb{P}$ with Radon-Nikodym derivation $p$~(w.r.t. a uniform measure $\nu$) on $(E, \Ecal)$, its \emph{Gibbs measure} w.r.t. a function $h: E\to\mathbb{R}$ is defined as a probability measure $\rho_h(\mathbb{P})$ which satisfies that
\begin{align*}
    \rho_h({\mathbb{P}})(A)\propto \mathbb{E}_{x^\prime\sim\mathbb{P}}[\mathbf{1}_{A}(x^\prime)e^{h(x^\prime)}].
\end{align*}

By Donsker and Varadhan's Variational Formula, for any $M\in\Mcal$ and $h: \Ocal\to\mathbb{R}$~(we will specify $h$ later), 
\begin{align*}
    \log\mathbb{E}_{\Dcal\sim M}[\exp(h(\Dcal))] = \sup_{\rho\in\Delta (\Ocal)}\Big[\mathbb{E}_{\Dcal\sim \rho}[h(\Dcal)]-\KL(\rho\rVert M)\Big]
\end{align*}
where the maximum is reached by the Gibbs measure $\rho_{M, h}$.
This means that 
\begin{align*}
    \log\mathbb{E}_{\Dcal\sim M}[\exp(h(\Dcal))] = \mathbb{E}_{\Dcal\sim \rho_{M, h}}[h(\Dcal)]-\KL(\rho_{M, h}\rVert M).
\end{align*}
By Jensen's inequality, we have that
\begin{align*}
    \mathbb{E}_{\Dcal\sim M}[h(\Dcal)] \le
    \log\mathbb{E}_{\Dcal\sim M}[\exp(h(\Dcal))] = \mathbb{E}_{\Dcal\sim \rho_{M, h}}[h(\Dcal)]-\KL(\rho_{M, h}\rVert M).
\end{align*}
For any algorithm $\mathfrak{A}$, we can assign $h$ as $\Lcal(M, \mathfrak{A}(\cdot))/4B$
and conclude that, for any $\mathfrak{A}$ and $M\in\Mcal$, 
\begin{align*}
    \mathbb{E}_{\Dcal\sim M}[\Lcal(M, \mathfrak{A}(\Dcal))] \le&\Big[\mathbb{E}_{\Dcal\sim \rho_{M, \mathfrak{A}}}[\Lcal(M, \mathfrak{A}(\Dcal))]-4B\cdot\KL(\rho_{M, \mathfrak{A}}\rVert M)\Big]\\\le&
    \sup_{\rho\in\Delta(\Ocal)}\Big[\mathbb{E}_{\Dcal\sim \rho}[\Lcal(M, \mathfrak{A}(\Dcal))]-4B\cdot\KL(\rho\rVert M)\Big]
\end{align*}
Taking $\inf_{\mathfrak{A}}\sup_{M\in\Mcal}$ in both sides yields that 
\begin{align*}
    \inf_{\mathfrak{A}}\sup_{M\in\Mcal}\mathbb{E}_{\Dcal\sim M}[\Lcal(M, \mathfrak{A}(\Dcal))] \le&
    \inf_{\mathfrak{A}} \sup_{M\in\Mcal}\sup_{\rho\in\Delta(\Ocal)}\Big[\mathbb{E}_{\Dcal\sim \rho}[\Lcal(M, \mathfrak{A}(\Dcal))]-4B\cdot\KL(\rho\rVert M)\Big].
\end{align*}
Meanwhile, by change of measure we have that
\begin{align*}
    \inf_{\mathfrak{A}}\sup_{M\in\Mcal}\mathbb{E}_{\Dcal\sim M}[\Lcal(M, \mathfrak{A}(\Dcal))]\ge
    &\frac{1}{3}\inf_{\mathfrak{A}}\sup_{M\in\Mcal}\sup_{\rho\in\Delta(\Ocal)}\Big[\mathbb{E}_{\Dcal\sim \rho}[\Lcal(M, \mathfrak{A}(\Dcal))]-4B\cdot\KL(\rho\rVert M)\Big].
\end{align*}
As a result, 
\begin{align*}
    \inf_{\mathfrak{A}}\sup_{M\in\Mcal}\mathbb{E}_{\Dcal\sim M}[\Lcal(M, \mathfrak{A}(\Dcal))]\simeq
    &\inf_{\mathfrak{A}}\sup_{M\in\Mcal}\sup_{\rho\in\Delta(\Ocal)}\Big[\mathbb{E}_{\Dcal\sim \rho}[\Lcal(M, \mathfrak{A}(\Dcal))]-4B\cdot\KL(\rho\rVert M)\Big]\\=&
    \inf_{\mathfrak{A}}\sup_{\rho\in\Delta(\Ocal)}\sup_{M\in\Mcal}\Big[\mathbb{E}_{\Dcal\sim \rho}[\Lcal(M, \mathfrak{A}(\Dcal))]-4B\cdot\KL(\rho\rVert M)\Big]
\end{align*}
\begin{align*}
    \sup_{\rho\in\Delta(\Ocal)}\inf_{\mathfrak{A}} \sup_{M\in\Mcal}\Big[\mathbb{E}_{\Dcal\sim \rho}[\Lcal(M, \mathfrak{A}(\Dcal))]-4B\cdot\KL(\rho\rVert M)\Big]\le&
    \sup_{\rho\in\Delta(\Ocal)}\inf_{p\in\Delta(\Pi)} \sup_{M\in\Mcal}\Big[\Lcal(M, p)-4B\cdot\KL(\rho\rVert M)\Big]\\=&
    \oec(\Delta(\Ocal), \Mcal).
\end{align*}
This completes the proof.


==> lemmas/tools.tex <==


\subsection{Reinforcement Learning}



\begin{lemma}[Simulation lemma, maybe we need episode version, cf. Lemma 9 in \citet{Uehara2021PessimisticMO}]
    \begin{align*}
        |J_M(\pi) - J_{M^\prime}(\pi)|\le V_{\max}\TV(M, M^\prime, d_{M, \pi})
    \end{align*}
\end{lemma}

\begin{proof}
    \begin{align*}
        &J_M(\pi) - J_{M^\prime}(\pi)\\=& 
        \mathbb{E}_{r_0\sim M(\pi), s_0\sim M(\pi)}\big[r_0+V_{M, \pi}(s_1)\big]-
        \mathbb{E}_{r_0\sim M^\prime(\pi), s_0\sim M^\prime(\pi)}\big[r_0+V_{M^\prime, \pi}(s_1)\big]\\=&
        \mathbb{E}_{r_0\sim M(\pi), s_0\sim M(\pi)}\big[r_0+V_{M^\prime, \pi}(s_1)\big]-
        \mathbb{E}_{r_0\sim M^\prime(\pi), s_0\sim M^\prime(\pi)}\big[r_0+V_{M^\prime, \pi}(s_1)\big]\\&\quad+
        \mathbb{E}_{s_1\sim M^\prime(\pi)}\big[V_{M, \pi}(s_1)-V_{M^\prime, \pi}(s_1)\big]\\\le&
        \mathbb{E}_{(s_0, a_0)\sim M(\pi)}\big[\Delta R(s_0, a_0) + V_{\max}\Delta P(s_0, a_0) \big]-
        \mathbb{E}_{s_1\sim M^\prime(\pi)}\big[V_{M, \pi}(s_0)-V_{M^\prime, \pi}(s_1)\big]\\\le&
        \mathbb{E}_{(s, a)\sim M(\pi)}\big[\Delta R(s, a)\big]+
        \mathbb{E}_{(s, a)\sim M(\pi)}\big[V_{\max}\Delta P(s, a) \big]
    \end{align*}
\end{proof}


==> lemmas/transfer1.tex <==
\begin{lemma-a}
    Given a measurable space $(\Omega, \mathcal{E})$, two probabilities $\mathbb{P}$ and $\mathbb{Q}$, and a positive number $\beta>0$, 
    for any real valued measurable function $f$ on $\Ecal$ with range $[0, \beta]$, 
    \begin{align*}
        \big|\mathbb{E}_{\mathbb{P}}[f] -\mathbb{E}_{\mathbb{Q}}[f]\big|
        \le2\beta\TV(\mathbb{P}, \mathbb{Q}).
    \end{align*}
\end{lemma-a}

\begin{proof}
    Take $\nu\coloneqq \mathbb{P}+\mathbb{Q}$ as the dominating measure, 
    we have that
    \begin{align*}
        \TV(\mathbb{P}, \mathbb{Q})=&\frac{\int\Big|\frac{d\mathbb{P}}{d\nu}-\frac{d\mathbb{Q}}{d\nu}\Big|d\nu}{2}\\=&
        \frac{\int\beta\Big|\frac{d\mathbb{P}(x)}{d\nu(x)}-\frac{d\mathbb{Q}(x)}{d\nu(x)}\Big|\nu(dx)}{2\beta}\\\ge&
        \frac{\int f(x)\Big|\frac{d\mathbb{P}(x)}{d\nu(x)}-\frac{d\mathbb{Q}(x)}{d\nu(x)}\Big|\nu(dx)}{2\beta}\\=&
        \frac{\int \Big|f(x)\frac{d\mathbb{P}(x)}{d\nu(x)}-f(x)\frac{d\mathbb{Q}(x)}{d\nu(x)}\Big|\nu(dx)}{2\beta}\\\ge&
        \tag{Jensen's inequality}
        \frac{\Big|\int \Big(f(x)\frac{d\mathbb{P}(x)}{d\nu(x)}-f(x)\frac{d\mathbb{Q}(x)}{d\nu(x)}\Big)\nu(dx)\Big|}{2\beta}\\=&
        \frac{\Big|\int \big(f(x)\frac{d\mathbb{P}(x)}{d\nu(x)}\big) \nu(dx)-\int\big(f(x)\frac{d\mathbb{Q}(x)}{d\nu(x)}\big)\nu(dx)\Big|}{2\beta}\\=&
        \frac{\big|\mathbb{E}_{\mathbb{P}}[f] -\mathbb{E}_{\mathbb{Q}}[f]\big|}{2\beta}\tag{\Cref{lemma:derivative}}
    \end{align*}
    The fifth inequality is due to Jensen's inquality and the fact that the absolute value function is convex.

    This completes the proof.
\end{proof}


==> sections/algo.tex <==
\section{F2D}

\IncMargin{1em}
\begin{algorithm}
\caption{F2D}\label{algo}
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{Dataset $\mathcal{D}$, MDPs class $\Mcal$}
Estimate best fit model $\hat{\Mcal}$
\begin{align*}
    \hat{\Mcal} = \{M\mid \mathbb{P}_M(\mathcal{D})\ge 1-\delta\}.
\end{align*}\\
Estimate the pessimissm policy
\begin{align*}
    \hat{\pi} = 
    \argmin\limits_{\pi\in\Pi}
    \max\limits_{M\in\hat{\Mcal}}
    \Delta J_{M}(\pi).
\end{align*}\\
\Output{$\hat{\pi}$}
\end{algorithm}\DecMargin{1em}

No empty since itself.

\subsection{Sample complexity via F2D}

We define 
\begin{align*}
\est(\Mcal)\coloneqq \max\limits_{M\in\hat{\Mcal}}\max\limits_{M^\prime\in\hat{\Mcal}} \TV(M, M^\prime).
\end{align*}
\begin{lemma}
    Given $\hat{\Mcal}\in\Mcal$, and $M^\star\in\hat{\Mcal}$, 
    \begin{align*}
    \Delta J_{M^\star}(\hat{\pi})
    \ge& \oec(\Mcal)+2V_{\max}\est(\hat{\Mcal}).
    \end{align*}
\end{lemma}

\begin{proof}
Fixing $\hat{\Mcal}$, $\hat{\pi}$ is no longer a random variable.

\begin{align*}
    J_{M^\star}(\hat{\pi})\ge&J_{M(\hat{\pi})}(\hat{\pi})\\=&
    \max\limits_{\pi\in\Pi}\min\limits_{M\in\hat{\Mcal}}J_{M}(\hat{\pi})\\\ge&
    \min\limits_{M^\prime\in\hat{\Mcal}}\max\limits_{\pi\in\Pi}\min\limits_{M\in\hat{\Mcal}}\Big[J_{M}(\hat{\pi})+2V_{\max}\TV(M, M^\prime)\Big]-2V_{\max}\est(\hat{\Mcal})\\\ge&
    \min\limits_{M^\prime\in\Mcal}\max\limits_{\pi\in\Pi}\min\limits_{M\in\Mcal}\Big[J_{M}(\hat{\pi})+2V_{\max}\TV(M, M^\prime)\Big]-2V_{\max}\est(\hat{\Mcal})\\=&
    \oec(\Mcal)-2V_{\max}\est(\hat{\Mcal})
\end{align*}
\end{proof}

\begin{remark}
    The introduced $\est$ term would be asymptoticly small since it depedend on 
    \begin{align*}
        \min\limits_{M\in\Mcal}
        \min\limits_{M^\prime\in\Mcal}\TV(M, M^\prime)
    \end{align*}
\end{remark}

\textcolor{red}{TODO: I beg you, do not use $\log\lvert\Mcal\rvert$}

\begin{lemma}
    with probability at least $1-\delta$, $M^\star\in\hat{\Mcal}$.
\end{lemma}

\begin{lemma}
    with probability at least $1-\delta$, $\est(\Mcal)\le$.
\end{lemma}

\begin{remark}
    Assuming $M^\star\in\Mcal$, $\Mcal$ should be as simple as possible.
    $\est$ would be small even the model is hard to learn, i.e., contains similar $M$ and $M^\prime$ with large deviation of $\Delta J$.
\end{remark}

\begin{theorem}
    \label{theorem:f2d}
    Assuming that hold, with probability at least $1-\delta$, 
    \begin{align*}
        J_M(\hat{\pi}) \ge \oec(\Mcal)-2V_{\max}\sqrt{\frac{\log(1/\delta)}{N}}
    \end{align*}
\end{theorem}

\begin{remark}
    While the lower bound and upper is not match perfectly, they shows the learnability.
\end{remark}


==> sections/concrete.tex <==
\section{Concrete}

There is no need to include actions.

\begin{table}[H]
  \centering
\begin{tabular}{c|cccc}
\toprule
$M$ & $0.5$ & $0.6$ & $0.7$ & \\
\midrule
 $\pi$ \\
 $1$ & $0.2$ & $0$ & $0.9$ &  \\
 $2$ & $0.8$ & $1$ & $0.1$ &  \\
\midrule
 $\mathfrak{A}$ &  &  &  &  max\\
$0, 1\to 1$ & $0.1$ & $0$ & $0.9$ & $0.9$ \\
$0, 1\to 2$ & $0.8$ & $1$ & $0.1$  & $1$ \\
$0/1\to 1/2$ & $0.5$ & $0.6$ & $0.34$  & $0.6$ \\
$0/1\to 2/1$ & $0.5$ & $0.4$ & $0.66$  & $0.66$ \\
\midrule
 $\Dcal$ &  &  &  & \\
 $0$ & $-0.3$ & $-0.6$ & $0.56$ & \\
 $1$ & $0.3$ & $0.4$ & $-0.24$ & \\
\bottomrule
\end{tabular}
\end{table}

\section{Extension}

Can we show that 
\begin{align*}
    \max_{M^\star\in\Mcal}\mathbb{E}_{\Dcal\sim M^\star}\Big[\min_{p\in\Delta(\Pi)}\max_{M\in\Mcal}\big[\Lcal(M, p)+\log(\mathbb{P}_{M}(\Dcal))-\log(\mathbb{P}_{M^\star}(\Dcal))\big]\Big]
\end{align*}
is a lower bound in some sense?
A note is that we have the lower bound 
\begin{align*}
    \max_{M^\star\in\Mcal}\min_{p\in\Delta(\Pi)}\max_{M\in\Mcal}\mathbb{E}_{\Dcal\sim M^\star}\Big[\Lcal(M, p)+\log(\mathbb{P}_{M}(\Dcal))-\log(\mathbb{P}_{M^\star}(\Dcal))\Big].
\end{align*}

Consider the case that we have the dataset $\Dcal$, what's the limitation of the bound.
The performance of algorithm depends on the underlying models.

\subsection{$\Dcal$}

One most normal thought would be taking some $M$, 

As the algorithm is minimax optimal, it would map $\Dcal$ to that $\pi$ even if it is more like that this dataset is generated by another $M$. This is the natural of the algorithm. But the problem is that, how can we find the algorithm that fit into this natural?

The existence of the algorithm can be justified, but the principal to find this is hard to be identified.

The two bounds cannot be fitted naturally since that we can easily find the counterexample.

Or this bound can always be achieved if we have unlimited computation power: we can iterate all possible algorithms and computes their maximum error. But this is not allowed and is to complex...

How to search this algorithm efficiently, or at least achieve a balance, it's a consistent goal.

The empirical divergence is optimal if it can characterize the performance of the minimax optimal algorithm.

As the discussion on properties and tightness reveals, 
this algorithmic bound should not be achieved by simply a log-likelihood. Or this may means that this characterize the algorithm difference.

But when in some cases, at the lost of some constants and log-terms?

A dumb decision may be directly taking the difference and stating the result. But most people would not buy this.


==> sections/model_free.tex <==
\section{Application to Model-free Functions}

\textcolor{red}{C. Mao-TODO: delete this?}

As , any assumption on model-free function classes is putting restriction on the underlying model class.

Generally speaking, decision making is centered with find the optimal decisions.
Note that the coverage assumptions is also 
We can obtain model class from the conditions we made

\begin{align}
    \hat{\pi}\coloneqq \argmin_{\pi\in\Pi} \max_{M\in\Mcal}\Big[\Lcal(M, \pi)-\lambda\cdot\lli(\Dcal, M, M^\star)\Big].
\end{align}

ED2 is a learning matter, 

\paragraph{On the Value Function Class} Each value function $q$ has a bunch of models admitting that $q$ is optimal.
The major barrier .


==> sections/new_rule.tex <==
\section{New Rule}

\begin{align*}
    D(M, M^\prime)\coloneqq \sup_{\mathfrak{A}}\mathbb{E}_{\Dcal\sim M, \Dcal^\prime\sim M^\prime}\Big[\Lcal(M^\prime, \mathfrak{A}(\Dcal^\prime))-\Lcal(M^\prime, \mathfrak{A}(\Dcal))\Big].
\end{align*}
Take 
\begin{align*}
    \hat{D}(M, M^\prime)\coloneqq \sup_{\mathfrak{A}}\mathbb{E}_{\Dcal^\prime\sim M^\prime}\Big[\Lcal(M^\prime, \mathfrak{A}(\Dcal^\prime))-\Lcal(M^\prime, \mathfrak{A}(\Dcal))\Big]
\end{align*}
where $\Dcal\sim M$.

Policy to models, 
\begin{align*}
    \Mcal(\pi, \epsilon)\coloneqq \{M| \Lcal(M, \pi)\le\epsilon\}.
\end{align*}
\textcolor{red}{C. Mao-TODO: There may be no model that performs such well.}
Models to policies, 
\begin{align*}
    \pi(\Mcal) \coloneqq \argmin_{\pi\in\Pi}\max_{M\in\Mcal} \Lcal(M, \pi).
\end{align*}

\begin{lemma}
    \begin{align*}
        \max_{M\in\Mcal}\Lcal(M, \pi(\Mcal(\pi, \epsilon)))\ge\max_{M\in\Mcal}\Lcal(M, \pi).
    \end{align*}
\end{lemma}

Take double min in oec.


==> sections/ope.tex <==
\section{Off-policy Evaluation}

We consider the 
In off-policy evaluation. There is a policy $\pi_{\texttt{ope}}$.
In this setting, the policy class is a class of value functions.
We takes the loss function as 
\begin{align*}
    \Lcal(M, q)=\lVert q-Q^{\pi_{\texttt{ope}}}\rVert_{2, \nu}.
\end{align*}

